Visualization for Epidemiological Modelling: Challenges, Solutions, Reflections & Recommendations

We report on an ongoing collaboration between epidemiological modellers and visualization researchers by documenting and reflecting upon knowledge constructs -- a series of ideas, approaches and methods taken from existing visualization research and practice -- deployed and developed to support modelling of the COVID-19 pandemic. Structured independent commentary on these efforts is synthesized through iterative reflection to develop: evidence of the effectiveness and value of visualization in this context; open problems upon which the research communities may focus; guidance for future activity of this type; and recommendations to safeguard the achievements and promote, advance, secure and prepare for future collaborations of this kind. In describing and comparing a series of related projects that were undertaken in unprecedented conditions, our hope is that this unique report, and its rich interactive supplementary materials, will guide the scientific community in embracing visualization in its observation, analysis and modelling of data as well as in disseminating findings. Equally we hope to encourage the visualization community to engage with impactful science in addressing its emerging data challenges. If we are successful, this showcase of activity may stimulate mutually beneficial engagement between communities with complementary expertise to address problems of significance in epidemiology and beyond. https://ramp-vis.github.io/RAMPVIS-PhilTransA-Supplement/

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> process-themes/process-scaleScope.tex <==
\subsubsectionALT{Scale \& Scope via Trial \& Error}
{The Scale and Scope through Trial and Error Strategy}
{Scale \& Scope via Trial \& Error}
\label{sub:scaleScope}
\label{sub:trialError}
\label{sub:trialerror}

The VIS literature is full of working examples of interactive graphics and systems and designs that have shown to be effective in particular contexts. But it is often unclear \textit{under which conditions} particular idioms apply.
%% Applied work such as the RAMP volunteering has an important contribution to make to help us refine our knowledge of the catalogue of potential solutions. 
%% We have shown that we worked closely with colleagues with complementary domain expertise to establish the effectiveness of possible visualizations solutions in a variety of use cases.
Determining whether plausible visualization solutions `fit' across tasks and data sets, whether they scale and transfer to the new context and scope, plays an important role in refining our knowledge of the catalogue of potential visual and analytic solutions to data problem-solving.
This was achieved repeatedly during rapid response through informed trial and error that relies upon an \textit{experimental} and \textit{analytical} perspective to the visualization design process (as described in sections \ref{sub:experiments} and \ref{sub:analysisisdesign}).
%%
%% It is essential to document the results of this thinking, the findings about `fit', to justify approaches used and document knowledge to support future efforts:
It enabled us to explore questions around scale and scope during transfer including:
how many data items can be used?
what kinds of data distributions (as well as data structures) may fit (or not fit)?
to which kinds of problems can this approach be (usefully) applied?

%% Applied work and applied settings such as those encountered during the RAMP volunteering have
%% an important role in refining our knowledge of the catalogue of potential visual and analytic solutions to data problem-solving.
For example, experimental learning through specific instances showed that: 
\begin{itemize}
  \setlength\itemsep{0.25em}
\item\obs{https://observablehq.com/d/4aebb875cacaef3a,669} certain techniques apply well to data sets with particular characteristics;
 \item\obs{https://observablehq.com/d/c3a628d8bd4fe8fe,733} pre-processing may be required in some cases due to data volumes;
 \item\obs{https://observablehq.com/d/43927395f6cb890c,596} conventional network techniques are ineffective;
 %% \noteM{JD}{Need animations link}
\obs{https://observablehq.com/d/43927395f6cb890c,596} animations with large numbers of changes are overwhelming
 \item\obs{https://observablehq.com/@kaimdx/rampvis-idiom-gmap,709} certain algorithms do not scale adequately to provide interactive speeds;
 \item\obs{https://observablehq.com/d/880d234e47a1ed24,438} particular views are sensitive to low level design choices involving alternative layouts and orderings
 or \obs{https://observablehq.com/@aidans/rampvis-idiom-gridded-glyphmaps,791} variations within the graphic such as different population densities across a map.
\end{itemize}

In a \textit{Critical Creative Culture} (\secref{sub:creativeCulture}) this can of course result in inspired thinking to refine approaches and produce viable new solutions, such as through the population-proportional fading used to account for population densities in our \textit{Gridded GlyphMaps} \obs{https://observablehq.com/@aidans/rampvis-idiom-gridded-glyphmaps,788}, that may in turn be of use elsewhere.

Comprehensive and systematic testing of the \textit{Scale \& Scope} (\secref{sub:scaleScope}) at which visual idioms apply
across a range of contexts and data sets would be very useful in the event of the kind of rapid response required during the COVID pandemic: 
particularly if this and their refinement are described and documented comprehensively and transparently (\secref{sub:documentdesign}).
Such activity can potentially reduce the reliance on, and bias inherent in, the \textit{Deep Dig} (\secref{sub:deepdig}). 

==> rampvis-authorInfo.V2.tex <==
\huge\textbf{CO-AUTHOR INSTRUCTIONS}

\vspace{12px}
\Large{\textbf{
\textcolor{Maroon}{Please read this cover page \& do what it says!}}
}
\vspace{12px}

\large{
We now have a full draft ready for submission. Most \textbf{MUST} and many \textbf{SHOULD} comments have been addressed and some of the narrative boiled down and focused -- hopefully adequately!

If you have already signed off - fine ... but we hope that you will additionally check through and sign off this final version over the next two days - by end of 12th Oct.
If we have an answer from you already -- \textbf{fine, we can take this} -- but here is a second opportunity to see the \textbf{final thing} and let us know whether you would like to :

\begin{itemize}
    \setlength{\itemsep}{0pt}%
    \item Remain listed as a \textbf{co-author} (we hope that you do!)
    \item Be removed from the author list but be \textbf{listed in the acknowledgments} for your contribution instead 
    \item Be \textbf{removed} entirely without acknowledgment
\end{itemize}

Evidently we hope that all co-authors will want to be associated with the work as authors - we have tried to make the paper representative of the views that have been expressed.
However, if the draft does not represent your views - please let us know, this could be useful feedback and we'd like to try to accommodate you if we can.
We would like everybody to be included, to agree with the thrust of the paper, and to have their contributions recognised.
But we also owe you the opportunity to opt out, and to have your say -- no questions asked if that's your preference!
}

\vspace{9px}
\LARGE{\textbf{State of the Draft - Ready to Submit}}

\vspace{6px}
\large{
We have improved things a little and hope to submit as close to this circulated draft as possible.

We'd like people to have a final read through to check for any errors or inconsistencies that \textbf{MUST} be addressed and \textbf{sign-off}.
}

\vspace{9px}
\LARGE{\textbf{\textcolor{Maroon}{What CO-AUTHORS Need To Do}}}

\vspace{6px}
\large{
We'd like you to \textbf{read through once}, completely, without making comments - to get a sense of the flow and the content and the claims and the coherence and whether you can sign off.
}

\vspace{6px}
\large{
Then we'd like you to let us know any issues that \textbf{MUST} BE ADDRESSED prior to publication. Each will take time. Please keep them to a minimum as the paper will not be perfect for anybody! But if you think it \textbf{MUST} be addressed, then please list it as a \textbf{MUST} and we will do our best.
We'd love to hear about errors, inaccuracies and important omissions.
}


\vspace{6px}
\large{
If anything has changed, or if you have not done so already, please \textbf{please fill in the \href{https://forms.gle/vV2uqQ3JJL4ovRvM8}{Google Form for Authors}}\\(\textit{click the bold text in the line above to go there!}).
}

\vspace{6px}
\large{
\textbf{Sub-Title} --
\textit{The paper is supposed to be on \textbf{Technical Challenges} so here are some options - my preference is for the final one - if you are \textbf{strongly against this}, please let me know! ...}\\
%%
 -- Technology, Techniques \& Teamwork\\
% \item Rapid Assistance in Visualizing the Pandemic\\
 -- Progress, Examples and Reflections on RAMP\\
 -- Problems, Progress and Priorities\\
 -- Technological, Analytical \& Organizational Challenges, Opportunities, Solutions \& Priorities\\
 -- Technologies, Challenges, Solutions \& Learning\\
 -- Progress, Priorities and Reflection on Rapid Assistance in the Pandemic\\
 -- \textbf{\textcolor{Maroon}{Challenges, Solutions, Reflections \& Recommendations}}
}


\vspace{9px}
\LARGE{\textbf{\textcolor{Maroon}{What IDIOM LEADS Need To Do}}}

\vspace{6px}
\large{
There are two unattributed quotes in the text!
Please have a look and let me know if these are in your idiom notebooks!


\begin{itemize}
    \item \textbf{sec 4.3} \sayIt{the idiom seems highly suited to COVID related analyses due to the complexities of the data points themselves and their limited number.  On the negative side the idiom is somewhat poorly explored in existing literature and there isn’t sufficient guidance and support for its deployment}
\end{itemize}


\begin{itemize}
    \item \textbf{sec~4.2} \sayIt{explore the use of the idiom in real analysis settings - how is it used, what analyses does it support, what are the scenarios that it maps to best}
\end{itemize}

Please make sure that your \textbf{idiom notebook} is clean and published.
\\ \\\textbf{FINAL DEADLINE : OCT 13th 5pm}\\ \\
These are our \textbf{data}, they will be seen by leading scientists, and we need to ensure that everything they see is complete and well-considered.
The more I think about the notion of updating data post submission, the less appropriate it seems.\\\textbf{Let's try to get the notebooks sorted before we submit on Wednesday please}.

Some of you have still not done the following ...
\begin{itemize}
    \setlength{\itemsep}{0pt}%
    \item Respond to comments and resolve them;
    \item Unpin the markdown;
    \item Break text up into small cells;
    \item Remove any content that is not for public consumption (and ensure that you have permission to publish the views and materials that are within the notebook);
\end{itemize} 

Please also \textbf{update the spreadsheet}. Make sure that your row is up to date. The columns with red headers are particularly important -- these are your columns that enable me to see what you have done -- and we need you to keep them current.
% We also need a \textbf{40 character summary} of each idiom to appear in Table \ref{tab:table-name}. \textbf{Please add this}.
}

\vspace{9px}
\LARGE{\textbf{Finally}}

\vspace{6px}
\large{
% The current status is unintentional, and to be honest, a bit of an embarrassment. But this is a big beast, and a tough job. Turning it around, wrangling it gently takes T--I--M--E.
% We probably underestimated the extent of the job. Sorry about that!

We are nearly there.

Sorry it has taken so long and been such a big job.

But please do as requested \textbf{promptly} to get us over the line.

We hope it's worth it and are pleased with the quality of documentation of our diverse collective efforts, the original meta-analysis and the key themes and recommendations.
}

\vspace{6px}
\large{
% So, on the minus side - you are being asked to sign off on something that is incomplete.
% But, on the plus side, we're on track with Plan V3 and you have the chance to influence things, a little.
% We hope that the plus outweighs the minus and that you are able to sign up!

% \vspace{6px}
Please act as requested in good time!

Thanks.

\vspace{6px}
\textbf{Jason \& Alfie, Cagatay, Min}
}






==> rampvis-authorInfo.tex <==
\huge\textbf{CO-AUTHOR INSTRUCTIONS}

\vspace{6px}
\large{
We promised a draft for you to sign off over the next two days - by end of 22nd Sept.
\textbf{This is it}.
It's not quite as complete as we had hoped.
But it should give you enough to know whether you would like to :

\begin{itemize}
    \setlength{\itemsep}{0pt}%
    \item Remain listed as a \textbf{co-author} (we hope that you do!)
    \item Be removed from the author list but be \textbf{acknowledged} instead 
    \item Be \textbf{removed} entirely without acknowledgment
\end{itemize}

Evidently we hope that all co-authors will want to be associated with the work as authors - we have tried to make the paper representative of the views that have been expressed.
However, if the draft does not represent your views - please let us know, this could be useful feedback and we'd like to try to accommodate you if we can.
We would like everybody to be included, to agree with the thrust of the paper, and to have their contributions recognised.
But we also owe you the opportunity to opt out, and to have your say -- no questions asked if that's your preference!
}

\vspace{9px}
\LARGE{\textbf{State of the Draft - Incomplete}}

\vspace{6px}
\large{
The paper is better following your feedback but it's too long, so it will need to have cuts and re-wordings. We hope that this will neither reduce the quality, scope, or examples and evidence. This should all remain pretty constant if we edit well.
}

\vspace{6px}
\large{
The paper contains some comments and discussion - these will be acted on, but this should give you a sense of where it is going.
The paper contains red summary sections.
These will be removed and we may add some signposting instead, but again, this should help you see what you are signing off on!
}

\vspace{9px}
\LARGE{\textbf{What CO-AUTHORS Need To Do}}

\vspace{6px}
\large{
We'd like you to \textbf{read through once}, completely, without making comments - to get a sense of the flow and the content and the claims and the coherence and whether you can sign off.
}

\vspace{6px}
\large{
Then we'd like you to let us know any issues that \textbf{MUST} BE ADDRESSED prior to publication. Each will take time. Please keep them to a minimum as the paper will not be perfect for anybody! But if you think it \textbf{MUST} be addressed, then please list it as a \textbf{MUST} and we will do our best.
We'd love to hear about errors, inaccuracies and important omissions.
}


\vspace{6px}
\large{
We'd then like to know any issues that \textbf{SHOULD} BE ADDRESSED prior to publication. No more than 2 or 3 please. We will resolve as many of these as we can (though there may be conflicts and time is limited). But let us know what \textbf{SHOULD} be done. This might include :
\begin{itemize}
    \setlength{\itemsep}{0pt}%
    \item repetition to remove
    \item candidates for cutting
    \item other general comments (and possible solutions)
    % \item repetition (joke)
\end{itemize}
}

\vspace{6px}
\large{
We don't want to know about issues that \textbf{COULD} BE ADDRESSED if we had more time or \textbf{WOULD} BE ADDRESSED if you were the only author and had forever! Time is short, changes are expensive. The time for these was yesterday!
}

\vspace{6px}
\large{
We do however  need some details from you, as requested by the journal - so \textbf{please fill in the \href{https://forms.gle/vV2uqQ3JJL4ovRvM8}{Google Form for Authors}}.
}

\vspace{9px}
\LARGE{\textbf{What IDIOM LEADS Need To Do}}

\vspace{6px}
\large{
We hope that all the idioms get a mention and that all mentions are appropriate. But, it turns out, this is a hard thing to manage and ensure in a dynamic document!

So we need your eyes on this. Please check for mentions of your idiom - check that they are there, and let us know if the idiom is missing or misrepresented.

Also, please \textbf{check your reflection} and see whether your idiom could add to any of the themes. There is still time to link evidence from the reflection in the notebooks to the claims and recommendations made in the paper.

If so, them please \textbf{add a comment starting with IDIOM}, \textbf{an explanation}, \textbf{the URL of the cell in the notebook} and \textbf{a short piece of text that links the two}. E.g.
}

\vspace{4px}
\small{My idiom does this through Wizard of Oz - see reflection here :\\
~\url{https://observablehq.com/@jwolondon/rampvis_idiom_odmap#cell-1328}\\
\textbf{ODMaps were refined and developed through `Wizard of Oz’ interaction} 
}

\vspace{6px}
\large{
Please also update the \textbf{idiom notebook}. These are our data, they will be seen by competent scientists, and we need to ensure that everything they see is complete and well-considered. The more I think about the notion of updating data post submission, the less appropriate it seems. \textbf{Let's try to get the notebooks sorted before we submit on Friday please}.
\begin{itemize}
    \setlength{\itemsep}{0pt}%
    \item Respond to comments and resolve them;
    \item Unpin the markdown;
    \item Break text up into small cells;
    \item Remove any content that is not for public consumption (and ensure that you have permission to publish the views and materials that are within the notebook);
\end{itemize} 

Please also \textbf{update the spreadsheet}. Make sure that your row is up to date. The rows with red headers are particularly important and we need you to keep them current. We also need a \textbf{40 character summary} of each idiom to appear in Table \ref{tab:table-name}. \textbf{Please add this}.
}

\vspace{9px}
\LARGE{\textbf{Finally}}

\vspace{6px}
\large{
The current status is unintentional, and to be honest, a bit of an embarrassment. But this is a big beast, and a tough job. Turning it around, wrangling it gently takes T--I--M--E.
We probably underestimated the extent of the job. Sorry about that!

}

\vspace{6px}
\large{
So, on the minus side - you are being asked to sign off on something that is incomplete.
But, on the plus side, we're on track with Plan V3 and you have the chance to influence things, a little.
We hope that the plus outweighs the minus and that you are able to sign up!

\vspace{6px}
Please act as requested in good time!\\Thanks.

\vspace{12px}
\textbf{Jason \& Alfie, Cagatay, Min}
}






==> rampvis-editorInfo.tex <==
\huge\textbf{RAMP VIS - DRAFT 1.3d}

\vspace{9px}
\LARGE{\textbf{NOTES FOR EDITORS}}

\vspace{12px}

\large{~\\
Hi - \\

thanks for the invitation to submit to the Theme Issue of PTRSA on \textit{Technical challenges of modelling real-life epidemics and examples
of overcoming these}. We have experienced plenty of these and show in the paper how \textit{Visualization Research} can be applied to address them and enhanced by doing so. 
Our manuscript follows and has been signed off by all 33 authors.\\

We are a little over the suggested word/page limit, but this is a large collaborative project and there is plenty to say, and doing so with credibility and authority requires plenty of evidence. As such we have produced a somewhat ambitious set of online supplementary materials and make frequent reference to these. You'll see the direct links from the manuscript to this evidence base. These are important in terms of narrative, methodology and provenance. We hope that you will be able to retain these direct links in the manner that we have included them here should the paper be accepted.\\

There is also plenty to show. The supplementary materials contain rich interactive examples of visualization, but we had to leave many interesting, informative and innovative graphics out of the paper due to the constraints that have been communicated. This is a shame as graphics and figures showcase visualization work particularly well. If there is any opportunity to add graphics should the paper be accepted for the \textit{Special Issue}, then we would be very pleased to do so - they show our work effectively and strengthen the arguments that we present. 
}

\vspace{9px}
\LARGE{\textbf{Contributions}}
\vspace{6px}

\large{
The 33 co-authors made significant contributions in \textbf{support}ing the project, the \textbf{volunteering} effort in which much of the work was undertaken, to \textbf{data} generation that enabled us to document our activity and establish claims, and in developing the \textbf{manuscript}, as follows ...
}

\vspace{9px}
\large{\textbf{SUPPORT}}
\vspace{3px}

%% SUPPORT
\large{
Alfie Abdul-Rahman,
Daniel Archambault,
Rita Borgo,
Min Chen,
Jason Dykes,
Hui Fang,
Nigel W. John,
Andrew Lahiff,
Robert S. Laramee,
Panagiotis Ritsos \&
Cagatay Turkay ...

provided \textbf{support} through project conceptualisation, administration, system support, resource provision (computing and other resources) and funding acquisition.
}

\vspace{9px}
\large{\textbf{VOLUNTEERING}}
\vspace{3px}

%% VOLUNTEERING
\large{
Alfie Abdul-Rahman,
Daniel Archambault,
Benjamin Bach,
Rita Borgo,
Min Chen,
Jason Dykes,
Jessica Enright,
Hui Fang,
Elif E. Firat,
Euan Freeman,
Tuna Gönen,
Radu Jianu,
Saiful Khan,
Louise Matthews,
Sibylle Mohr,
Phong H. Nguyen,
Alma Rahat,
Panagiotis Ritsos,
Jonathan C. Roberts,
Aidan Slingsby,
Ben Swallow,
Thomas Torsney-Weir,
Cagatay Turkay,
Franck Vidal,
Qiru Wang,
Jo Wood \&
Kai Xu ...

were involved in \textbf{volunteering} - modelling, visualization, analysis, reporting and reflection as described in the Observable notebooks.
}

\vspace{9px}
\large{\textbf{DATA}}
\vspace{3px}

%% DATA
\large{
Alfie Abdul-Rahman,
Daniel Archambault,
Rita Borgo,
Min Chen,
Jason Dykes,
Jessica Enright,
Elif E. Firat,
Euan Freeman,
Tuna Gönen,
Radu Jianu,
Saiful Khan,
Sibylle Mohr,
Phong H. Nguyen,
Richard Reeve,
Panagiotis Ritsos,
Aidan Slingsby,
Cagatay Turkay,
Franck Vidal,
Qiru Wang,
Jo Wood \&
Kai Xu ...

generated \textbf{data} - creating, commenting on, discussing, and developing the evidence base presented in the Observable notebooks.
}

\vspace{9px}
\large{\textbf{MANUSCRIPT}}
\vspace{3px}

%% MANUSCRIPT
\large{
Alfie Abdul-Rahman,
Daniel Archambault,
Rita Borgo,
Min Chen,
Jason Dykes,
Radu Jianu,
Nigel W. John,
Jonathan C. Roberts,
Aidan Slingsby,
Ben Swallow,
Cagatay Turkay,
Jo Wood \&
Kai Xu ...

contributed to the \textbf{manuscript} - through writing, critical review, commentary and revision of paper drafts through which claims, narrative and conclusion were developed.
}

\vspace{9px}
\LARGE{\textbf{Keywords}}
\vspace{6px}

\large{
We suggest the following:
\begin{itemize}
    \setlength{\itemsep}{0pt}%
    \item Visualization
    \item Visual Analytics
    \item Epidemiological Modelling
\end{itemize}
}



\vspace{9px}
\LARGE{\textbf{Source}}
\vspace{6px}

\large{
The manuscript is described in \textit{LaTeX} using \textit{Overleaf} and we would of course be happy to provide the source should this be useful at any stage. 
Just let us know.

We can provide individual figure files (PNG or other) for production as requested in the \textit{Information for Authors}. 
}

\vspace{9px}
\LARGE{\textbf{Supporting Data}}
\vspace{6px}

\large{
Our \textit{Supporting Data} are the \textit{Observable} notebooks. 
These are publicly accessible online and detailed in the reference list.
We can arrange for them to be uploaded to \textit{figshare} or \textit{Dryad} if required.
They point to other (large) open data sets that have been generated through the SCRC volunteering.
}

\vspace{36px}
\begin{flushright}
\large{
\textbf{Prof. Jason Dykes,}\\
City, University of London.\\
Lead and Corresponding Author\\
j.dykes@city.ac.uk\\
\textit{15th October, 2021}.
}
\end{flushright}


==> rampvis-test.tex <==
%% Testing LaTeX

\section{Testing Links}

We make direct reference to evidence in these notebooks by citing with \textbf{cite} through URL keys \cite{https://observablehq.com/@jwolondon/rampvis_idiom_odmap} that give us inline links in the paper directly to cells in our evidence base

We use \textbf{cell} to link directly to cells in the notebook, for example when demonstrating the utility of applying numeric and graphical transformations to reveal structure \cell{https://observablehq.com/@jwolondon/rampvis_idiom_odmap}{2072}.
%%
This seems to work well.
%%
Here is another example \cell{https://observablehq.com/d/54c8641168c013ea}{699}.

\subsection{obs}
Two arguments -- \obs{https://observablehq.com/d/54c8641168c013ea,699}.\\
One argument -- \obs{https://observablehq.com/d/54c8641168c013ea}.

